A novel segmented-scintillator antineutrino detector

The next generation of very-short-baseline reactor experiments will require compact detectors operating at surface level and close to a nuclear reactor. This paper presents a new detector concept based on a composite solid scintillator technology. The detector target uses cubes of polyvinyltoluene interleaved with $^6$LiF:ZnS(Ag) phosphor screens to detect the products of the inverse beta decay reaction. A multi-tonne detector system built from these individual cells can provide precise localisation of scintillation signals, making efficient use of the detector volume. Monte Carlo simulations indicate that a neutron capture efficiency of over 70% is achievable with a sufficient number of $^6$LiF:ZnS(Ag) screens per cube and that an appropriate segmentation enables a measurement of the positron energy which is not limited by gamma-ray leakage. First measurements of a single cell indicate that a very good neutron-gamma discrimination and high neutron detection efficiency can be obtained with adequate triggering techniques. The light yield from positron signals has been measured, showing that an energy resolution of 14%/$\sqrt{E({\mathrm{MeV}})}$ is achievable with high uniformity. A preliminary neutrino signal analysis has been developed, using selection criteria for pulse shape, energy, time structure and energy spatial distribution and showing that an antineutrino efficiency of 40% can be achieved. It also shows that the fine segmentation of the detector can be used to significantly decrease both correlated and accidental backgrounds.

==> SoLidTech-Arxiv 2/SoLid_author_list_templateStyle.tex <==
%This file is included in main document by using "\input{SoLid_author_list}"

%Something to allow multiple use of same footnote
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

%Institutes: with short name as new command
\address[a]{Universiteit Antwerpen, Antwerpen, Belgium}
\address[b]{University of Bristol, Bristol, UK}
\address[c]{Vrije Universiteit Brussel, Brussel, Belgium}
\address[d]{LPC Caen, ENSICAEN, Universit\'e de Caen, CNRS/IN2P3, F-14050 Caen, France}
\address[e]{CERN, 1211 Geneva 23, Switzerland}
\address[f]{Universiteit Gent, Gent, Belgium}
\address[g]{Imperial College London, Department of Physics, London, United Kingdom}
\address[h]{SUBATECH, CNRS/IN2P3, Universit\'e de Nantes, Ecole des Mines de Nantes, Nantes, France}
\address[i]{LAL, Univ Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay, France}
\address[j]{University of Oxford, Oxford, UK}
\address[k]{SCK-CEN, Belgian Nuclear Research Centre, Mol, Belgium}
\address[l]{Center for Neutrino Physics, Virginia Tech, Blacksburg, Virginia, 24061, USA}
\address[m]{STFC, Rutherford Appleton Laboratory, Harwell Oxford, and Daresbury Laboratory, Warrington, United Kingdom}

%List of authors and their corresponding institute
\author[a]{Y.~Abreu \footnote{\label{ceaden} on leave from CEADEN, Havana, Cuba}}
\author[i]{Y.~Amhis}
\author[b]{L.~Arnold}
\author[d]{G.~Ban}
\author[a]{W.~Beaumont}
\author[i]{M.~Bongrand}
\author[i]{D.~Boursette}
\author[h]{J.~M.~Buhour}
\author[j]{B.~C.~Castle}
\author[b]{K.~Clark}
\author[k]{B.~Coup\'e}
\author[h]{A.~S.~Cucoanes \footnote{\label{roma} now at ELI-NP, Horia Hulubei National institute of Physics and Nuclear Engineering, Bucharest, Romania}}
\author[b]{D.~Cussans}
\author[a,e]{A.~De Roeck}
\author[c]{J.~D'Hondt}
\author[d]{D.~Durand}
\author[h]{M.~Fallot}
\author[h]{S.~Fresneau}
\author[k]{L.~Ghys}
\author[h]{L.~Giot}
\author[d]{B.~Guillon}
\author[h]{G.~Guilloux}
\author[g]{S.~Ihantola}
\author[a]{X.~Janssen}
\author[k]{S.~Kalcheva}
\author[c]{L.N.~Kalousis}
\author[k]{E.~Koonen}
\author[f]{M.~Labare}
\author[d]{G.~Lehaut}
\author[k]{J.~Mermans}
\author[f]{I.~Michiels}
\author[f,k]{C.~Moortgat}
\author[b,m]{D.~Newbold}
\author[l]{J.~Park}
\author[b]{K.~Petridis}
\author[a]{I.~Pi\~nera \footnoteref{ceaden}}
\author[b]{G.~Pommery}
\author[k]{L.~Popescu}
\author[h]{G.~Pronost}
\author[b]{J.~Rademacker}
\author[j]{A.~Reynolds}
\author[f]{D.~Ryckbosch}
\author[j]{N.~Ryder}
\author[b]{D.~Saunders}
\author[g]{Yu.~A.~Shitov}
\author[i]{M.-H.~Schune}
\author[j]{P.~R.~Scovell}
\author[i]{L.~Simard}
\author[g]{A.~Vacheret \footnote{\label{author} Corresponding author}} \ead{antonin.vacheret@imperial.ac.uk}
\author[k]{S.~Van Dyck}
\author[c]{P.~Van Mulders}
\author[a]{N.~van Remortel}
\author[a,c]{S.~Vercaemer} 
\author[j]{A.~Waldron}
\author[j,m]{A.~Weber}
\author[h]{F.~Yermia}
